Big Graph Search: Challenges and Techniques

On one hand, compared with traditional relational and XML models, graphs have more expressive power and are widely used today. On the other hand, various applications of social computing trigger the pressing need of a new search paradigm. In this article, we argue that big graph search is the one filling this gap. To show this, we first introduce the application of graph search in various scenarios. We then formalize the graph search problem, and give an analysis of graph search from an evolutionary point of view, followed by the evidences from both the industry and academia. After that, we analyze the difficulties and challenges of big graph search. Finally, we present three classes of techniques towards big graph search: query techniques, data techniques and distributed computing techniques.

==> sec-subgraphsearch.tex <==
\section{Graph Search}
\label{sec-gsearch}

\,Graph search is kind of query language executing on graphs. Namely, given a input graph G, it outputs
subgraphs of G satisfying some specific semantic requirements. We will next introduce three types of graph
search: cohesive subgraphs, keyword search on graphs and graph pattern matching.\par

\subsection{Cohesive Subgraph}
\label{subsec-cohesive}
\,Cohesive subgroup originally indicates subgroup of actors among whom there exist relatively strong or intense ties
within a network. Different cohesive subgroups are formed according to different cohesive relations, which are
further specified by application needs. As mentioned above, social networks can be represented as graphs, so
that we formalize cohesive subgroups as cohesive subgraphs. Correspondingly, the problem of searching for cohesive
subgraphs in a graph is referred to as cohesive subgraph search.\par
\,Here we will mainly introduce some common types of cohesive subgraphs, by using the famous "Padgett's Florentine
Families" example (Fig.~\ref{fig-padgettfamily}) for explanation~\cite{Wasserman94}. The family network includes marriage and business ties among 16 historical
prominent families in the 15th century Florence, and following we will only analyze marriage ties. In the
network graph, a node denotes a family labeled with family name, and an edge exists between a pair of nodes if a
member in one family marries a member in another family. In the ancient days, marital ties could be used to
solidify political and economic alliances, such that by finding out the alliances using cohesive subgraph
technologies, scientists can learn and study the history of 15th century Florence conveniently and comprehensively,
while focusing on political and economic relations among the alliances~\cite{Wasserman94}. \par

\begin{figure}
  % Requires \usepackage{graphicx}
  \vspace{1.5ex}
  \begin{center}
  \includegraphics[scale=0.8]{./padgettfamily.eps}\\
  \end{center}
  \vspace{-4.5ex}
  \caption{Padgett's Florentine family}\label{fig-padgettfamily}
  \vspace{-3ex}
\end{figure}

\textbf{Maximal clique:} A maximal clique in a graph is a maximal complete subgraph with at least three nodes. The nodes
in a clique are adjacent to each other, and there are no other nodes that are also adjacent to all of the members
in the clique. In "Padgett's Florentine Families", there exist three maximal cliques, they are:\par
 	$\bullet$ $\text{n}_4$:Bischer, $\text{n}_{11}$:Peruzzi and  $\text{n}_{15}$:Strozzi,\par
 	$\bullet$  $\text{n}_5$:Castellani,  $\text{n}_{11}$:Peruzz and $\text{n}_{15}$:Strozzi,\par
 	$\bullet$ $\text{n}_9$:Medici, $\text{n}_{13}$:Ridolfi and $\text{n}_{16}$:Tornabuoni.\par
\, Due to the excellent mathematical properties and closed structure characters the clique has, it has provided a foundation for studying cohesive subgroups in social network. However, the definition of clique is so restrict that substantively there are always such few cliques exist satisfying the rules in a graph. In addition, the size of the clique is generally limited by the degree of the nodes within it. We could find that there are only three maximal cliques and each only has three nodes in "Padgett's Florentine Families".\par
\, In practical applications, to make the result more universal, a common idea to extend the definition for maximal clique arises, by weakening the restrictions for resulting subgraphs, such as n-clique, n-clan and k-clique etc.\par

\textbf{N-clique:} An n-clique in a graph is a maximal subgraph in which the largest distance between any two nodes is no
greater than n. The definition is less restrictive than the one for clique, since it only requires each pair of nodes in an n-clique
should be reachable but not necessarily adjacent, such that the n-cliques found in a graph are generally both larger and more numerous
than the cliques found in the graph. For example, there are thirteen 2-cliques in "Padgett's Florentine Families". For the reason that the definition of n-clique
does not make restrictions on how to calculate the distance, therefore, the diameter(the maximum distance between any pairwise nodes)
of the subgraph may be larger than n. For instance, the diameter of the 2-clique consists of five families
($\text{n}_{2}$:Albizzi, $\text{n}_{4}$:Bischer, $\text{n}_{7}$:Guadagni, $\text{n}_{13}$:Ridolfi, $\text{n}_{16}$:Tornabuoni) is 3, which is
larger than 2. That is because the \textcolor{red}{diameter path} connecting a pair of nodes in an n-clique may contain nodes that
lie outside the n-clique. Thus, the structure of n-clique is not as cohesive as expected originally.\par

\textbf{N-clan:}  An n-clan is an n-clique in which the diameter is no greater than n. Intuitively, to make the structure of
cohesive subgraph more cohesive, n-clan makes a further restriction based on n-clique, requiring that the diameter of an n-clique
should be no greater than n. Namely, all the nodes included in the \textcolor{red}{diameter path} should lie inside the n-clique.\par

\textbf{K-core:} A k-core in a graph is a maximal subgraph with each nodal degree no smaller than k. For example, in "Padgett's Florentine Families", there exists one 2-core containing ten families.\par
 	$\bullet$ $\text{n}_{2}$:Albizzi, $\text{n}_{3}$:Barbadori, $\text{n}_{4}$:Bischeri, $\text{n}_{5}$:Castellani, $\text{n}_{7}$:Guadagni, $\text{n}_{9}$:Medici, $\text{n}_{11}$:Peruzzi, $\text{n}_{13}$:Ridolfi, $\text{n}_{15}$:Strozzi and $\text{n}_{16}$:Tornabuoni.\par
\,With the cohesive relations gradually looser (compared with maximal clique, the restrictions for n-clique and n-clan are weaker),
we could find that by extending the definitions gradually, the resulting subgraphs satisfying the rules are generally both larger and more numerous.
In addition, it is an NP hard problem to find maximum subgraphs in a graph, such that maximal clique, n-clique and n-clan haven't adopt
the maximum subgraph semantic, which is actually a compromise on considering the balance between the accuracy of query results and
query efficiency. Finally, for k-core, the semantics of maximal and maximum subgraph are equal, and can be both solved in polynomial time.

\subsection{Keyword Search on Graphs}

\, Nowadays, with the popularity of information technology and the development of Internet, we could find an obvious growth in data amount. Subsequently, a problem arises, how to retrieve desired information in such large amount of data resources, which becomes a hot topic in research field. "Keyword Search" makes it possible searching for information from data resources for users. Furthermore, due to its simple but user-friendly interface, keyword search is virtually the information retrieval mechanism for data on Internet.\par
\, Moreover, it proves to be effective to execute keyword search on graphs. Given a data graph and a set of keywords, generally, nodes in a data graph are labeled with some keywords. Keyword search is to search for subgraphs of which the nodes containing the input keywords and satisfying some specific structural constraints. Therefore, the nodes structure and the content contained in nodes are both concerned in the search, of which the basic requirement is to find subgraphs with nodes containing all the input keywords. Different search methods and techniques are produced according to different structural constraints, and then we will introduce three types of keyword search methods on graphs.\par
\textbf{Minimum Spanning Tree:} Most keyword search methods take the minimum spanning tree semantic. It is to search for a tree with all the input keywords appearing in the nodes of the tree, and the total weight of all the edges in the tree is minimum.\par
\textbf{R-Radius Steiner Graph:} Given a graph $G$ with radius no more than r and a keyword set $Q$, if two nodes $u$ and $v$ in $G$ directly contain one or some input keywords in $Q$ individually, all the nodes on the path between $u$ and $v$ (including $u$ and $v$) in $G$ are called Steiner nodes~\cite{GuoliangLi08}. The subgraph of $G$ composed of Steiner nodes and associated edges is called an r-radius Steiner graph. In nature, Steiner node is kind of node that directly or indirectly contains one or some input keywords in $Q$. The subgraph of $G$ composed of Steiner nodes and associated edges is called an r-radius Steiner graph, such that the output result of keyword search is an r-radius Steiner graph~\cite{Aggarwal10}.\par

\begin{figure}
  \vspace{1.5ex}
  \begin{center}
  \includegraphics[scale=0.5]{./keywordsearch.eps}\\
  \end{center}
  \vspace{-4.5ex}
  \caption{The process of keyword search on graphs}\label{fig-keyword}
  \vspace{-3ex}
\end{figure}

\textbf{R-clique:} This method outputs result organized as r-clique (as mentioned in section~\ref{subsec-cohesive}), with the node collection containing all the input keywords, and the distance between any pair of nodes in the
collection is no larger than r, which makes a restriction on the cohesive relation of the keyword search result~\cite{Mehdi11}. The process
of executing keyword search on graphs with r-clique semantic is depicted in Fig.~\ref{fig-keyword}. Firstly, the user assigns and enters a set of
keywords \{A, B, C\} into the system; then by performing keyword search on the data graph in database, it retrieves a collection of subgraphs ${G'_1, G'_2,..., G'_k}$ containing
the input keywords from data graph; finally, the system would rank the subgraphs according to some specific ranking methods. For instance,
$G'_2$ is ranked before $G'_1$ as the connection between its root and matches is even tighter.

\, Actually, due to the lack of structural constraints among keywords when executing keyword search on graphs, to "guess" the structural topology of keywords is generally necessary, which has formed a variety of keyword search semantics. Therefore, the query process requires a combination of ranking based on the supposing of users' expectations, after obtaining the keyword search results. Consequently, keyword search methods (including classic keyword search methods) are usually combined with ranking techniques.\par

\subsection{Graph Pattern matching}
\, Graph pattern matching plays an increasingly important role in social network. The formal definition is as below.
Given two directed graphs $G_1$ (pattern graph) and $G_2$ (data graph), graph pattern matching is to (1) decide
whether $G_1$ "matches" $G_2$ (Boolean queries); or (2) identify "subgraphs" of $G_2$ that match $G_1$.\par
\, Graphs here are composed of node set and edge set, with labels on the nodes and edges identifying some relevant information.
The definition for graph pattern matching includes two categories of queries. The first type is boolean query that the answer
is either "Yes" or "No", and the results of the second one are based on the first one.
In addition, pattern graphs are generally relatively small, only containing several or dozens of nodes. On the contrary, data graphs
are usually larger, as the number of nodes contained in a data graph has reached hundred millions orders of magnitude\textcolor{green}{~\cite{ShuaiMaCCF12}}. As we know,
different "matching" semantics generate different matching languages, even though they take the same graph as pattern graph,
such as subgraph isomorphism~\cite{Ullmann76}, graph simulation~\cite{FanLMTWW10} and strong simulation~\cite{ShuaiMaVLDB12} etc.\par

\textbf{Graph Isomorphism:} Given a data graph $G$ and a pattern graph $Q$, graph isomorphism of $Q$ and $G$ is a bijection $f$ from
the nodes in $Q$ to the nodes in $G$ such that (1) for each pattern node $u$ in $Q$, $u$ and $f(u)$ have the same label, and (2) there exists
an edge $(u, v)$ in $Q$ if and only if ($f$(u), $f$(v)) is an edge in $G$.\par
\textbf{Subgraph Isomorphism:} Given a data graph $G$ and a pattern graph $Q$, a subgraph isomorphism problem is to determine whether
$G$ contains a subgraph that is isomorphic to $Q$. \par
\, We will next introduce graph pattern matching by the example of recommender systems in section~\ref{sec-app}. We can take $G$ and $Q$ in Fig.~\ref{fig-recommendation} as
data graph and pattern graph. Then by executing graph pattern matching on $G$, we could find that $G$ and $Q$ are not matched via the semantic
of subgraph isomorphism. That is, there exist no subgraphs in $G$ who have exactly the same structural topology with $Q$.\par
\, As we know, graph pattern matching is an NP-complete problem, which comes the lower query efficiency,
and in certain scenarios, the structural topology requirements are too restrictive to find matches in a data graph. All of that hinder
its usability in emerging applications, such as social network. Hence, recent researches are aiming at improving the usability
of graph pattern matching in emerging applications by reducing or weakening the constraints of subgraph isomorphism. There are
mainly two ways: one possible method is to propose novel matching models, such as graph simulation, strong simulation and so on; the other is to
make use of approximate matching semantic. We will next make a general introduction to graph simulation and strong simulation.\par

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[tb!]
\vspace{-1ex}
\begin{center}
\begin{small}
\hspace*{-2ex}
\begin{tabular}{| c || c |c|c|c|c|c||c|}
\hline
\textbf{Matching}& \textbf{children}&\textbf{parents}&\textbf{connectivity}&\textbf{cycles}&\textbf{locality}
&\textbf{matches}&\textbf{Bisimilar\&b'ed-cycle}\\
\hline
$\eps$    & $\checkmark$ & $\times$& $\times$ & $\checkmark$ (directed), $\times$ (undirected)&
 $\times$  & $\times$ & $\times$ \\
\hline
$\deps$   &  $\checkmark$& $\checkmark$& $\checkmark$ & $\checkmark$ (directed \& undirected)
& $\times$ & $\times$ & $\times$ \\
\hline
$\dleps$  &  $\checkmark$& $\checkmark$& $\checkmark$ & $\checkmark$ (directed \& undirected)&
$\checkmark$ & $\checkmark$ & $\times$ \\
\hline
 $\iso$   &   $\checkmark$& $\checkmark$& $\checkmark$& $\checkmark$ (directed \& undirected)&
$\checkmark$ & $\times$ & $\checkmark$\\
\hline
\end{tabular}
\end{small}
\end{center}
\vspace{-3ex} \caption{Topology preservation and bounded matches}\label{tab-property}
\vspace{-4ex}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Graph simulation:} To reduce the complexity, graph simulation~\cite{FanLMTWW10} has been adopted for pattern matching, which can be determined in quadratic time.
A data graph $G$ matches a pattern graph $Q$ via graph simulation if there exists a binary relation $S \subseteq \text{V}_Q \times$ V ,
where $\text{V}_Q$ and V are the set of nodes in $Q$ and $G$, respectively, such that (1) for each $(u, v) \in S$, $u$ and $v$ have
the same label; and (2) for each node $u$ in $Q$, there exists $v$ in $G$ such that (a) $(u, v) \in S$, and (b) for each edge
$(u, u')$ in $Q$, there exists an edge $(v, v')$ in $G$ such that $(u', v') \in S$. Intuitively, graph simulation preserves labels and
child relationships of a graph pattern in its match, such that the definition for graph simulation is less restrictive than the one
sfor subgraph isomorphism. Simulation was initially proposed for the analysis of programs, and recently were
introduced for social network. In Fig.~\ref{fig-recommendation}, when simulation is adopted, all four biologists in $G$ are matches for Bio in
$Q$, and the entire data graph $G$ is included in match relation. However, $\text{Bio}_1$ and $\text{Bio}_2$ are recommended by either
HR only or by SE only in $G$, and $\text{Bio}_3$ is
recommended by neither an HR nor an SE. Only $\text{Bio}_4$ satisfies all these conditions that may be a candidate the headhunter wants.\par
\, Obviously, low complexity comes with a loss of accuracy in query results. Simulation and its extensions [19, 18] often
fall short in capturing the topology of data graphs, only returning a single matched subgraph, of which the match relation $S$ is
often too large to understand and analyze. It is necessary finding a balance between complexity and the capability to
capture topology. To achieve the goal, strong simulation has been developed.\par

\textbf{Strong simulation:} Strong simulation~\cite{ShuaiMaVLDB12}is a revision of graph simulation, by enforcing two conditions: (a)the duality to
preserve both child and parent relationships, while simulation considers only child relationships. We refer it as
dual simulation. (b) the locality to restrict matches within a ball of a certain radius. Considering the example in Fig.~\ref{fig-recommendation} again,
the subgraph of $G$ consists of $\text{HR}_2, \text{SE}_2, \text{Bio}_4, \text{AI}'_1, \text{AI}'_2, \text{DM}'_1$ and $\text{DM}'_2$
is the match of $Q$ via strong simulation, while $\text{Bio}_4$ is exactly the one that the headhunter wants to find.\par
\, We have also identified a set of criteria for topology preservation, and proved that strong simulation preserves the topology
between pattern graphs and data graphs. Based on the criteria, we then evaluate subgraph isomorphism, graph simulation, dual simulation
and strong simulation, as illustrated in Table~\ref{tab-property}. We use $Q \triangleleft G$ indicating that $G$ matches $Q$ via subgraph isomorphism.
%Data graph $G$ matches pattern graph $Q$ via subgraph isomorphism, denoted by $Q \triangleleft G$.
Similarly, $\prec$, $\prec_D$ and $\prec_D^L$ denote graph simulation, dual simulation and strong simulation respectively. \par
\, The property (1) children and (2) parents are criteria on measuring whether the semantic can preserve child or parent relationships.
Property (3) connectivity guarantees that a connected pattern graph only matches a connected subgraph in the data graph. Property (4)cycles
indicates that an undirected (resp. directed) cycle in $Q$ must match an undirected (resp. directed) cycle in $G$. Property (5)locality
requires the diameter of a matched subgraph in $G$ must be bounded by a function in the size of the pattern graph. Property (6)matches
indicates that there should be a bounded number of matches, and each match is small enough to inspect.

